Data-Oblivious Stream Productivity

We are concerned with demonstrating productivity of specifications of infinite streams of data, based on orthogonal rewrite rules. In general, this property is undecidable, but for restricted formats computable sufficient conditions can be obtained. The usual analysis disregards the identity of data, thus leading to approaches that we call data-oblivious. We present a method that is provably optimal among all such data-oblivious approaches. This means that in order to improve on the algorithm in this paper one has to proceed in a data-aware fashion.

==> pspackages.tex <==

\input{packages}
\input{macros.def}

\usepackage{pstricks}
\usepackage{pst-node}

\psset{arrowsize=4pt 2, arrowinset=0, labelsep=2pt, linewidth=0.1ex}

\newcommand{\arrowhead}[2]{ \ncput[nrot=:U,npos=1]{\rput(#1,#2){\psline[linestyle=solid](-0.235,-0.08)(-0.015,0)(-0.235,0.08)}} }
\newcommand{\psarrow}[3][]{ \ncline{#2}{#3} \arrowhead{0}{0} }
\newcommand{\psarrowd}[3][]{ \psarrow[#1]{#2}{#3} \arrowhead{-0.15}{0} }

\newcommand{\pseqh}{\nbput[npos=0.9,labelsep=0.15cm]{$=$}}
\newcommand{\pseqv}{\naput[npos=0.9,labelsep=0.10cm]{$=$}}

\newcommand{\labelP}{\pebnfbtrslab}%
\newcommand{\labelF}{\snetfb}%


